Visual Reference Resolution using Attention Memory for Visual Dialog

Visual dialog is a task of answering a series of inter-dependent questions given an input image, and often requires to resolve visual references among the questions. This problem is different from visual question answering (VQA), which relies on spatial attention (a.k.a. visual grounding) estimated from an image and question pair. We propose a novel attention mechanism that exploits visual attentions in the past to resolve the current reference in the visual dialog scenario. The proposed model is equipped with an associative attention memory storing a sequence of previous (attention, key) pairs. From this memory, the model retrieves the previous attention, taking into account recency, which is most relevant for the current question, in order to resolve potentially ambiguous references. The model then merges the retrieved attention with a tentative one to obtain the final attention for the current question; specifically, we use dynamic parameter prediction to combine the two attentions conditioned on the question. Through extensive experiments on a new synthetic visual dialog dataset, we show that our model significantly outperforms the state-of-the-art (by ~16 % points) in situations, where visual reference resolution plays an important role. Moreover, the proposed model achieves superior performance (~ 2 % points improvement) in the Visual Dialog dataset, despite having significantly fewer parameters than the baselines.

==> NIPS 2017 Camera Ready/sections/abstract.tex <==
% !TEX root = ../nips_2017.tex

\begin{abstract}
    Visual dialog is a task of answering a series of inter-dependent questions given an input image, and often requires to resolve visual references among the questions.
    This problem is different % iated 
    from visual question answering (VQA), which relies
    % relying 
    on spatial attention ({\em a.k.a. visual grounding}) estimated from % a pair of 
    an image and question pair. % alone.
    We propose a novel attention mechanism that exploits visual attentions in the past to resolve the current reference in the visual dialog scenario.
    The proposed model is equipped with an associative attention memory storing a sequence of previous (attention, key) pairs. 
    From this memory, the model retrieves the previous attention, taking into account recency, which is most relevant for the current question, in order to resolve potentially ambiguous references. 
    The model then merges the retrieved attention with a tentative one to obtain the final attention for the current question; specifically, we use dynamic parameter prediction to combine the two attentions conditioned on the question. Through extensive experiments on a new synthetic visual dialog dataset, we show that our model significantly outperforms the state-of-the-art (by $\approx 16$ \% points) in situations, where visual reference resolution plays an important role.
    Moreover, the proposed model achieves superior performance ($\approx 2$ \% points improvement) in the Visual Dialog dataset~\cite{visdial}, despite having significantly fewer parameters than the baselines.
%    While resolving visual reference is known to be useful for answering visually grounded questions, ambiguous expressions caused by the sequential dependency of questions in a dialog make it difficult to correctly resolve the references of the questions in the given image.
%    %The ambiguous expressions are used because of the shared contexts including the previous references between speakers.
%    In this paper, we propose a novel attention mechanism that uses previous visual references to resolve the current reference in the visual dialog scenario.
%    The proposed model is equipped with an attention memory storing previous attentions to handle the sequential dependency of visual expressions.
%    From the memory, the model retrieves a previous attention that has a dependency with the current reference based on their semantics.
%    The model merges the retrieved attention with the instantaneous attention that is newly calculated to obtain the final attention for the current reference.
%    We use dynamic parameter prediction to combine the two attentions differently based on the question.
%    Through exhaustive experiments on a synthetic visual dialog dataset, we show that our model is very strong in the situation where the visual reference resolution plays important roles.
%    Moreover, the proposed model also shows strong performances in real visual dialog dataset even with a smaller number of activations for sentence embeddings than the baselines.
\end{abstract}


% Visual dialog is a task of answering a series of inter-dependent questions given an input image. 
% This process often requires one to resolve visual references among the questions.
% This problem is different from visual question answering (VQA), which relies on spatial attention (a.k.a. visual grounding) estimated from an image and question pair.  
% We propose a novel attention mechanism that exploits visual attentions in the past to resolve the current reference in the visual dialog scenario.
% The proposed model is equipped with an associative attention memory storing sequence of previous (attention, key) pairs. 
% From this memory, the model retrieves previous attention, taking into account recency, that is most relevant for the current question, in order to resolve potentially ambiguous reference(s). 
% The model then merges the retrieved attention with the tentative one to obtain the final attention for the current question; specifically, we use dynamic parameter prediction to combine the two attentions conditioned on the question.
% Through exhaustive experiments on a new synthetic visual dialog dataset, we show that our model significantly outperforms the state-of-the-art (by $\approx 50$ \% points) in the situation where the visual reference resolution plays important role.
% Moreover, the proposed model presents superior performance ($\approx 2$ \% points improvement) in the Visual Dialog dataset, despite having significantly fewer parameters than the baselines.

==> NIPS 2017 Camera ready/sections/attmem.tex <==
% !TEX root = ../nips_2017.tex

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{./figures/network_architecture.pdf}
    \caption{{\bf Architecture of the proposed network.} The gray box represents the proposed attention process. Refer to Section~\ref{attmem} for the detailed description about individual modules (a)-(f).}
    \label{fig:network_architecture}
    \vspace{-0.1in}
\end{figure}

\section{Visual Dialog Model with Attention Memory-based Reference Resolution}
% \section{Reference Resolution with Attention Memory}
\label{attmem}
Visual dialog is the task of building an agent capable of answering a sequence of questions presented in the form of a dialog.
Formally, we need to predict an answer $y_t \in \mathcal{Y}$, where $\mathcal{Y}$ is a set of discrete answers or a set of natural language phrases/sentences, at time $t$ given input image $I$, current question $q_t$, and dialog history $H=\left\{h_\tau | ~h_\tau=\left(q_\tau, y_\tau\right),~0 \le \tau \lt t\right\}$.

We utilize the encoder-decoder architecture recently introduced in \cite{visdial}, which is illustrated in Figure~\ref{fig:network_architecture}. 
Specifically, we represent a triplet $(q,H,I)$ with $\bm{e}_t$ by applying three different encoders, based on recurrent (RNN with long-short term memory units), hierarchical recurrent (HRNN)\footnote{The questions and the answers of a history are independently embedded using LSTMs and then fused by a \texttt{fc} layer with concatenation to form QA encodings.
The fused QA embedding at each time step is finally fed to another LSTM and the final output is used for the history encoding.} and convolutional (CNN) neural networks, followed by attention and fusion units  (Figure~\ref{fig:network_architecture} (a)-(f)). 
Our model then decodes the answer $y_t$ from the encoded representation $\bm{e}_t$ (Figure~\ref{fig:network_architecture} (g)). Note that, to obtain the encoded representation $\bm{e}_t$, the CNN image feature map $\bm{f}$ computed from $I$ undergoes a soft spatial attention process guided by the combination of $q_t$ and $H$ as follows:
%
\iffalse
\begin{equation}
    \bm{f}^\mathrm{att} = [ \bm{\alpha}_t(\bm{c}_t) ]^\top \cdot \bm{f} = \sum^{N}_{n=1}{\alpha_{t,n}(\bm{c}_t) \cdot \bm{f}_n}, ~~\text{where}~~\bm{c}_t = \text{\texttt{fc}}(\text{RNN}(q_t), \text{HRNN}(H)), % = \sum^{N}_{t=1}{\alpha_t(c_t) \cdot f_t}, \label{attfeat}.
\end{equation} 
\fi
\begin{align}
\bm{c}_t &= \text{\texttt{fc}}(\text{RNN}(q_t), \text{HRNN}(H)) \\    
\bm{f}^\mathrm{att}_t &= [ \bm{\alpha}_t(\bm{c}_t) ]^\top \cdot \bm{f} = \sum^{N}_{n=1}{\alpha_{t,n}(\bm{c}_t) \cdot \bm{f}_n},
\end{align} 
%
%where $\bm{f}_n$ is a feature vector at the location $n$, $N$ is the size of the spatial grid of the feature map and $\bm{c}_t$ is a fused encoding of $q_t$ and $H$ obtained using a fully connected layer $\text{\texttt{fc}}$ (Figure~\ref{fig:network_architecture} (d)).
where $\text{\texttt{fc}}$ (Figure~\ref{fig:network_architecture} (d)) denotes a fully connected layer,  $\bm{\alpha}_n(\bm{c}_t)$ is the attention map conditioned on a fused encoding of $q_t$ and $H$, $n$ is the location index in the feature map, and $N$ is the size of the spatial grid of the feature map.
%Intuitively, the region of the image feature $n$ would contribute to the final answer proportionally to $\bm{\alpha}_n(\bm{c}_t)$. 
This attention mechanism is the critical component that allows the decoder to focus on relevant regions of the input image; it is also the main focus of this paper.

We make the observation that, for certain questions, attention can be resolved directly from $\bm{c}_t$.
This is called {\em tentative attention} and denoted by $\bm{\alpha}^\mathrm{tent}_t$. This works well for questions like \#1 in Figure~\ref{fig:md_ex}, which are free from dialog referencing. 
For other questions like \#6, resolving reference linguistically would be difficult (\eg linguistic resolution may look like: `What number of the digit to the left to the left of the brown 9'). 
%{\color{blue}[Given a sequence of questions indefinite reference, could be resolved to a definite reference, using co-reference resolution, for example. Purely based on NLP. This is what I tried to show in the example. However, than that resolved linguistic reference would need to be grounded in an image, i.e., the algorithm would need to know how to ground `to the left to the left of the brown 9'.]}
That said, \#6 is straightforward to answer if the attention utilized to answer \#5 is retrieved. 
This process of visual reference resolution gives rise to attention retrieval $\bm{\alpha}^\mathrm{mem}_t$ from the memory.
%Since both $\bm{\alpha}^\mathrm{tent}_t$ and $\bm{\alpha}^\mathrm{mem}_t$ are useful and complementary, 
The final attention $\bm{\alpha}_t(\bm{c}_t)$ is computed using dynamic parameter layer, where the parameters are conditioned on $\bm{c}_t$. 
To summarize, an attention is composed of three steps in the proposed model: tentative attention, relevant attention retrieval, and dynamic attention fusion as illustrated in Figure~\ref{fig:attention_process}.
%\ref{fig:attention_process}. 
We describe the details of each step below.




% As initially proposed in \cite{visdial}, the basic model inherits the encoder-decoder structure; multi-modal inputs are embedded using the encoder and the embedded representation is then decoded to generate answers.
% %{\color{red}We preserve the decoder structure of the previous model~\cite{visdial} as it changes depending on the evaluation settings. [I don't understand this sentence.]}
% While the proposed model adopts the same decoder architecture of \cite{visdial}, this section presents our encoder model, which is employed to embed images depending on spatial attention to visual references of linguistic inputs, \ie question and dialog history.



% \subsection{Attention-based Encoder}
% %describe with reference resolution
% The proposed encoder is based on the soft-attention model that has been adopted in multiple VQA models~\cite{askAtt,stackAtt,snuAtt,compQA,NMN,hierATT}.
% %As in these models, the proposed encoder computes an attention map highlighting the spatial region corresponding to the expression of an input question.
% %The computed attention map contains attention probabilities of individual locations in a feature map, which represent how much the corresponding features are relevant to the input question within the dialog.
% As in these models, the proposed encoder computes attention probabilities of individual locations in a feature map highlighting the spatial region corresponding to the expression of an input question.
% Once the attention map $\alpha$ is obtained, the attended feature $f^\mathrm{att}$ is then computed from the image feature map $\bm{f}$ as
% \begin{equation}
%     f^\mathrm{att} = \sum^{N}_{n=1}{\alpha_n f_n},  \label{attfeat}
% \end{equation}
% where $f_n\in \bm{f}$ is a feature vector at the location $n$ and $N$ is the size of the spatial dimension of the feature map.
% Note that noisy attention probabilities result in a noisy attended feature because the feature in each location is weighted by the corresponding attention probability; accurate estimation of attention probabilities is crucial for the attention-based encoder.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.58\linewidth}
\centering
\includegraphics[width=1\linewidth] {./figures/attention_process.pdf}
\caption{Dynamic combination of attentions}
\label{fig:attention_process}
%\centerline{(a) Dynamic combination of attentions}
\end{subfigure}
~~~~~~~~ 
\begin{subfigure}[b]{0.35\linewidth}
\centering
\includegraphics[width=1\linewidth] {./figures/memory_retrieval.pdf}
\caption{Attention retrieval from memory}
\label{fig:memory_retrieval}
%\centerline{(b) Attention retrieval from memory}
\end{subfigure}
\caption{
{\bf Attention process for visual dialog task.}
(a) The tentative and relevant attentions are first obtained independently and then dynamically combined depending on the question embedding.
(b) Two boxes represent memory containing attentions and corresponding keys. 
Question embedding $\bm{c}_t$ is projected by $\bm{W}^\mathrm{mem}$ and compared with keys using inner products, denoted by crossed circles, to generate address vector $\bm{\beta}_t$.
The address vector is then used as weights for computing a weighted average of all memory entries, denoted by $\Sigma$ within circle, to retrieve memory entry $\left(\bm{\alpha}^\mathrm{mem}_t, \bm{k}^\mathrm{mem}_t\right)$.
}
\label{fig:attention}
\vspace{-0.1in}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \subsection{Resolving Visual References}
% In visual dialog, it is challenging to estimate clear attention due to ambiguous referring expressions.
% %To alleviate this limitation, the proposed model employs a visual reference resolution module with an attention memory to access the previous references that are relevant to the ambiguous expressions. 
% %Note that ambiguous referring expressions are used with a dependency to a previous reference already shared between speakers.
% To alleviate this limitation, the proposed model employs a visual reference resolution module with an attention memory to access the relevant previous references as ambiguous referring expressions are used in a dependency to a previous reference already shared between speakers. 
% %{\color{red} [I don't understand.] Note that the ambiguous expressions are used when the references of the expressions are previously referred to.}
% Computation of attention maps is composed of three steps in the proposed model: instantaneous attention computation, relevant reference retrieval, and dynamic attention manipulation as illustrated in Figure~\ref{fig:attention_process}.
% We describe the details of each step below.

\subsection{Tentative Attention}
We calculate the tentative attention by computing similarity, in the joint embedding space, of the encoding of the question and history, $\bm{c}_t$, and each feature vector, $\bm{f}_n$, in the image feature grid ${\bm{f}}$: 
% in the image feature map after projecting them into a common semantic space.
%To resolve the visual reference of a question, we calculate an instantaneous attention based on the semantics of the question embedding and each feature in the image feature map.
%The question embedding and each image feature are first projected into a common semantic space and compared by the dot product.
% More precisely, the direct attention map $\alpha^\mathrm{dir}_t$ is computed over the image feature map $\bm{f}$ given the question embedding $c_t$ at time $t$ by 
\begin{align}
    s_{t,n} &= \left(\mathbf{W}^\mathrm{tent}_c \bm{c}_t\right)^\top \left(\mathbf{W}^\mathrm{tent}_f \bm{f}_n\right) \\
    \bm{\alpha}^\mathrm{tent}_{t} &= \mathrm{softmax}\left( \{ s_{t,n}, 1 < n < N \} \right),
\end{align}
where $\mathbf{W}^\mathrm{tent}_c$ and $\mathbf{W}^\mathrm{tent}_f$ are projection matrices for the question and history encoding and the image feature vector, respectively, and $s_{t,n}$ is an attention score for a feature at the spatial location $n$. 

%Although this attention map computed from the question embedding is known to be effective in VQA~\cite{askAtt,stackAtt,snuAtt,compQA,NMN} where each input question contains all the necessary information to answer, it is hard to obtain a clean attention map if the question contains ambiguities on referring the target visual concepts.
%Such ambiguities on the visual references can be managed by properly handling the dependency to the previous references.

\subsection{Relevant Attention Retrieval from Attention Memory}

As a reminder, in addition to the tentative attention, our model obtains the most relevant previous attention using an attention memory for visual reference resolution. 
%  as ambiguous expressions refer to some references that are already referred in the dialog history.
%As the ambiguities in the referring expressions are mainly because of the sequential dependency of references in dialogs, the proposed model keeps track of the previous references using an attention memory and retrieves the most relevant previous attention to the current question.

\paragraph{Associative Attention Memory}
The proposed model is equipped with an associative memory, called an attention memory, to store previous attentions.
The attention memory $\bm{M}_t = \left\{\left(\bm{\alpha}_0, \bm{k}_0\right), \left(\bm{\alpha}_1, \bm{k}_1\right), \dots, \left(\bm{\alpha}_{t-1}, \bm{k}_{t-1}\right)\right\}$ stores all the previous attention maps $\bm{\alpha}_\tau$ with their corresponding keys $\bm{k}_\tau$ for associative addressing.
Note that ${\bm{\alpha}_0}$ is \texttt{NULL} attention and set to all zeros. % with its corresponding key $k_0$.
The \texttt{NULL} attention can be used when no previous attention reference is required for the current reference resolution. 

The most relevant previous attention is retrieved based on the key comparison as illustrated in Figure~\ref{fig:memory_retrieval}.
%\ref{fig:memory_retrieval}.
Formally, the proposed model addresses the memory given the embedding of the current question and history $\bm{c}_t$ using
\begin{align}
    m_{t,\tau} = \left(\bm{W}^\mathrm{mem} \bm{c}_t\right)^\top \bm{k}_\tau
    ~~~~ \text{and} ~~~~
    \label{addressing}
    \bm{\beta}_t = \mathrm{softmax}\left( \{ m_{t,\tau} , 0 < \tau < t-1 \}\right),
\end{align}
where $\bm{W}^\mathrm{mem}$ projects the question and history encoding onto the semantic space of the memory keys.
The relevant attention $\bm{\alpha}^\mathrm{mem}_t$ and key $\bm{k}^\mathrm{mem}_t$ are then retrieved from the attention memory using the computed addressing vector $\bm{\beta}_t$ by
%
\begin{equation}
    \bm{\alpha}^\mathrm{mem}_t = \sum^{t-1}_{\tau=0}{\bm{\beta}_{t,\tau}\bm{\alpha}_\tau}\text{~~~~~~~and~~~~~~~~} \bm{k}^\mathrm{mem}_t = \sum^{t-1}_{\tau=0}{\bm{\beta}_{t,\tau} \bm{k}_\tau}.
\end{equation}
%
This relevant attention retrieval allows the proposed model to resolve the visual reference by indirectly resolving coreferences~\cite{coref1,coref2,coref3} through the memory addressing process.

\vspace{-0.1in}
\paragraph{Incorporating Sequential Dialog Structure}
While the associative addressing is effective in retrieving the most relative attention based on the question semantics, we can improve the performance by incorporating sequential structure of the questions in a dialog.
%While the associative addressing of the memory is effective to retrieve the relevant attentions, the addressing can be improved by incorporating with the sequential structure of dialogs.
%Note that the attention memory is an unordered set and is addressed purely based on the semantics of the keys.
Considering that more recent attentions are more likely to be referred again, we add an extra term to Eq.~(\ref{addressing}) that allows preference for sequential addressing, \ie
% \begin{equation}
    $m_{t,\tau}' = \left(\bm{W}^\mathrm{mem} \bm{c}_t\right)^\top \bm{k}_\tau + \theta \left(t-\tau\right)$
%    \label{seq_pref}
%\end{equation}
where $\theta$ is a learnable parameter weighting the relative time distance $(t-\tau)$ from the current time step.



\subsection{Dynamic Attention Combination}
After obtaining both attentions, the proposed model combines them.
The two attention maps $\bm{\alpha}^\mathrm{tent}_t$ and $\bm{\alpha}^\mathrm{mem}_t$ are first stacked and fed to a convolution layer to locally combine the attentions.
After generating the locally combined attention features, it is flattened and fed to a fully connected (\texttt{fc}) layer with softmax generating the final attention map.
However, a \texttt{fc} layer with fixed weights would always result in the same type of combination although the merging process should, as we argued previously, depend on the question.
Therefore, we adopt the dynamic parameter layer introduced in~\cite{DPPNet} to adapt the weights of the \texttt{fc} layer conditioned on the question at test time.
Formally, the final attention map $\bm{\alpha}_t(\bm{c}_t)$ for time $t$ is obtained by
\begin{align}
    \bm{\alpha}_t(\bm{c}_t) =  \mathrm{softmax}\left(\bm{W}^\mathrm{DPL}\left(\bm{c}_t\right) \cdot \gamma (\bm{\alpha}^\mathrm{tent}_t, \bm{\alpha}^\mathrm{mem}_t) \right),
\end{align}
where $\bm{W}^\mathrm{DPL}(\bm{c}_t)$ are the dynamically determined weights % by $c_t$ 
and $\gamma (\bm{\alpha}^\mathrm{tent}_t, \bm{\alpha}^\mathrm{mem}_t)$ is the flattened output of the convolution obtained from the stacked attention maps. 
%As in~\cite{DPPNet}, we use a hashing technique for the dynamic parameters to manage the large number of the parameters.
As in~\cite{DPPNet}, we use a hashing technique to predict the dynamic parameters without explosive increase of network size.
% With this final attention map $\alpha_t$ for time $t$, the encoding of the inputs $f^\mathrm{att}_t$ is calculated following equation~(\ref{attfeat}).

%\hsseo{would it be possible to add some theoretical proof of conv+DPP can handle any kind of transformation?}


==> NIPS 2017 Camera ready/sections/conclusion.tex <==
% !TEX root = ../nips_2017.tex

\section{Conclusion}
\vspace{-0.1in}
%\paragraph{Conclusions:}
We proposed a novel algorithm for answering questions in visual dialog.
Our algorithm resolves visual references in dialog questions based on a new attention mechanism with an attention memory, where the model indirectly resolves coreferences of expressions through the attention retrieval process.
We employ the dynamic parameter prediction technique to adaptively combine the tentative and retrieved attentions based on the question.
We tested on both synthetic and real datasets and illustrated improvements. 

\iffalse
We proposed a new attention mechanism for resolving visual references in dialog questions, using % by facilitating an 
attention memory. % for visual dialog.
The model resolves visual references by indirectly resolving coreferences of expressions through the attention retrieval process.
We also utilize the dynamic parameter prediction technique to dynamically combine the tentative and retrieved attentions based on the question.
We tested on both synthetic and real datasets and illustrate improvements. 
% of visual dialog and showed the proposed model outperforms the state-of-the-art baselines. 
\fi

==> NIPS 2017 Camera ready/sections/experiments.tex <==
% !TEX root = ../nips_2017.tex

\section{Experiments}
\vspace{-0.2cm}
We conduct two sets of experiments to verify % the  capability of 
the proposed model.
To highlight the model's ability to resolve visual references, % resolution, 
we first perform experiment % the model
with a synthetic dataset that is explicitly designed to contain ambiguous expressions and strong inter-dependency among questions in the visual dialog.
We then %, we 
show that the model % actually 
also works well in the real VisDial~\cite{visdial} benchmark.



\subsection{MNIST Dialog Dataset}

\paragraph{Experimental Setting}
We create
% We conduct experiments on 
a synthetic dataset, called MNIST Dialog\footnote{The dataset is available at \url{http://cvlab.postech.ac.kr/research/attmem}}, which is designed for the analysis of models in the task of visual reference resolution with ambiguous expressions.
Each image in MNIST Dialog contains a $4\times4$ grid of MNIST digits and each MNIST digit in the grid has four randomly sampled attributes, \ie $\mathrm{color}=\left\{\mathrm{red, blue, green, purple, brown}\right\}$, $\mathrm{bgcolor}=\left\{\mathrm{cyan, yellow, white, silver, salmon}\right\}$, $\mathrm{number}=\left\{x|0\le x\le9\right\}$ and $\mathrm{style}=\left\{\mathrm{flat, stroke}\right\}$, as illustrated in Figure~\ref{fig:md_ex}.
Given the generated image from MNIST Dialog,
% Given the image of a MNIST grid, 
we automatically generate questions and answers about a subset of the digits in the grid that focus on visual reference resolution.
%A question is either a counting question or an attribute question where the former asks the number of digits belonging to a subset and the latter asks an attribute of a single target digit.
There are two types of questions: (i) counting questions and (ii) attribute questions that refer to a single target digit.
% A question asks either the number of digits belonging to a subset or an attribute of a single target digit.
During question generation, the target digits for a question is selected based on a subset of the previous targets referred to by ambiguous expressions, as shown in Figure~\ref{fig:md_ex}.
For ease of evaluation, we generate a single word answer rather than a sentence for each question and there are a total of 38 possible answers ($\frac{1}{38}$ chance performance).
%(See Appendix A for more details of the generation.)
We generated 30K / 10K / 10K images 
for training / validation / testing, respectively, and three ten-question dialogs %with ten \leon{questions} 
for each image.

The % number of activations
dimensionality 
of the word embedding % layers 
and the hidden state in the LSTMs are set to 32 and 64, respectively. All LSTMs are single-layered.
Since answers are single words, the answer embedding RNN is replaced with a word embedding layer in both the history embedding module and the memory key generation module.
The image feature extraction module is formed by stacking four $3\times3$ convolutional layers with a subsequent $2\times2$ pooling layer.
The first two convolutional layers have 32 channels, % activations 
while there are 64 channels in the last two.
Finally, we use 512 weight candidates to hash the dynamic parameters of the attention combination process.
The entire network is trained end-to-end by minimizing the cross entropy of the predicted answer \mbox{distribution at every step of the dialogs.}

We compare our model (AMEM) with three different groups of baselines.
The simple baselines show the results of using statistical priors, where answers are obtained using % toward certain answers given 
image (I) or question (Q) only.
We also implement the late fusion model (LF), the hierarchical recurrent encoder with attention (HREA) and the memory network encoder (MN) introduced in \cite{visdial}.
Additionally, an attention-based model (ATT), which directly uses tentative attention, without memory access, is implemented as a strong baseline. % for this task.
For some models, two variants are implemented: one using history embeddings and the other one not.
These variations give us insights on the effect of using history contexts and are distinguished by +H.
Finally, another two versions of the proposed model, orthogonal to the previous ones, are implemented with and without the sequential preference in memory addressing (see above), which is denoted by +SEQ.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
    \begin{subfigure}[m]{0.37\linewidth}
        \centering
        \scalebox{0.8}{
            \begin{tabular}[b]{
               @{}C{1.7cm}@{}@{}C{0.4cm}@{}@{}C{0.7cm}@{}@{}C{1.1cm}@{}@{}C{0.3cm}@{}@{}C{1.6cm}@{}
            }
                Basemodel          	    && +H            & +SEQ          && Accuracy 		\\ \toprule
                I                 	    && --            & --            && 20.18			\\
                \multirow{2}{*}{Q}      && --            & --            && 36.58			\\ 
                                        && \checkmark    & --            && 37.58			\\ \cmidrule(lr){1-6}
                LF \cite{visdial}	    && \checkmark    & --            && 45.06			\\
                HRE \cite{visdial}	    && \checkmark    & --            && 49.10 		    \\
                MN \cite{visdial}	    && \checkmark    & --            && 48.51			\\ \cmidrule(lr){1-6}
                \multirow{2}{*}{ATT}    && --            & --            && 62.62			\\
                                        && \checkmark    & --            && 79.72			\\ \cmidrule(lr){1-6}
                \multirow{4}{*}{AMEM}   && --            & --            && 87.53			\\
                          	            && \checkmark    & --            && 89.20			\\
                    	                && --            & \checkmark    && 90.05			\\
                      	                && \checkmark    & \checkmark    && \bf96.39		\\ \bottomrule
            \end{tabular}
        }
    \end{subfigure}~~~~ %
    \begin{subfigure}[m]{0.6\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/turn_acc.pdf}
    \end{subfigure}
    \vspace{-0.05in}
    \caption{
        {\bf Results on MNIST Dialog.} Answer prediction accuracy [\%] of all models for all questions (left) and accuracy curves of four models at different dialog steps (right).
        +H and +SEQ represent the use of history embeddings in models and addressing with sequential preference, respectively.
    }
    \vspace{-0.1in}
    \label{fig:MDIAL_results}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\vspace{-0.2cm}
\paragraph{Results}
Figure~\ref{fig:MDIAL_results} shows the results on MNIST Dialog.
The answer prediction accuracy over all questions of dialogs is presented in the table on the left.
It is noticeable that the models using attention mechanisms (AMEM and ATT) significantly outperform the previous baseline models (LF, HRE and MN) introduced in \cite{visdial}, while these baselines still perform better than the simple baseline models.
This signifies the importance of 
attention
% the reference resolution 
in answering questions, consistent with
% as discovered in 
previous works \cite{NMN,compQA,askAtt,stackAtt,snuAtt}.
Extending ATT to incorporate history embeddings during attention map estimation increases the accuracy by about 17\%, resulting in a strong baseline model.

\vspace{-0.05cm}
However, even the simplest version of the proposed model, which does not use history embeddings or addressing with sequential preference, already outperforms the strong baseline by a large margin.
Note that this model still has indirect access to the history through the attention memory, although it does not have direct access to the encodings of past question/answer pairs when computing the attention.
% Note that this model is still capable of dealing with reference histories through the attention memory although it does directly not use the history embeddings in the attention calculation.
This signifies that the use of the attention memory is more helpful in resolving the current reference (and computing attention), compared to a method that uses more traditional tentative attention informed by the history encoding.
Moreover, the proposed model with history embeddings further increases the accuracy by 1.7\%.
The proposed model reaches >96\% accuracy when the sequential structure of dialogs is taken into account by the sequential preference in memory addressing.
% Moreover, the proposed model can be extended to use the history embeddings and the use of the history embeddings in the proposed model increases the accuracy by ~1.7 \%p.
% Finally, the proposed model even reaches over 96 \% of accuracy when the sequential structure of dialogs is taken into account by the sequential preference in the memory addressing.

\vspace{-0.05cm}
We also present the accuracies of the answers at each dialog step for four models that use attentions in Figure~\ref{fig:MDIAL_results} (right).
Notably, the accuracy of ATT drops very fast as the dialog progresses and reference resolution is needed.
Adding history embeddings to the tentative attention calculation somewhat reduces the degradation.
% of the accuracies at later steps of dialogs.
The use of the attention memory gives a very significant improvement, particularly at later steps in the dialog when complex reference resolution is needed.
% on the accuracies at later steps and our full model shows very stable performances at every step of dialogs.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\linewidth]{figures/beta.pdf}
    \caption{
    {\bf Memory addressing coefficients with and without sequential preference.}
    Both models put large weights on recent elements (smaller relative time difference) to deal with the sequential structure of dialogs.
    }
    \vspace{-0.1in}
    \label{fig:memory_addressing}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/tsne.pdf}
    \caption{
    {\bf Characteristics of dynamically predicted weights for attention combination.} 
    Dynamic weights are computed from 1,500 random samples at dialog step 3 and plotted by t-SNE.
    Each figure presents clusters formed by different semantics of questions. 
    (left) Clusters generated by different question types.
    (middle) Subclusters formed by types of spatial relationships in attribute questions. 
    (right) Subclusters formed by ways of specifying targets in counting questions; 
    cluster {\small\textsf{sub\_targets}} contains questions whose current target digits are included in the targets of the previous question.}
    \vspace{-0.1in}
    \label{fig:dpp_tsne}
\end{figure}

\paragraph{Parameter Analysis}
When we observed the learned parameter $\theta$ for the sequential preference, it is consistently negative in all experiments; it means that all models prefer recent elements. A closer look at the addressing coefficients $\bm{\beta}_t$ with and without the sequential preference reveals that both variants have a clear preferences for recent elements, as depicted in Figure~\ref{fig:memory_addressing}. 
It is interesting that the case without the bias term shows a stronger preference for recent information, but its final accuracy is lower than the version with the bias term.
It seems that $\bm{W}^\mathrm{mem}$ without bias puts too much weight on recent elements, resulting in worse performance.
Based on this observation, we learn $\bm{W}^\mathrm{mem}$ and $\theta$ jointly to find better coefficients than $\bm{W}^\mathrm{mem}$ alone.

The dynamically predicted weights form clusters with respect to the semantics of the input questions as illustrated in Figure~\ref{fig:dpp_tsne}, where 1,500 random samples at step~3 of dialogs are visualized using t-SNE.
In Figure~\ref{fig:dpp_tsne} (left), the two question types (attribute and counting) create distinct clusters. 
Each of these, in turn, contains multiple sub-clusters formed by other semantics, as presented in Figure~\ref{fig:dpp_tsne} (middle) and (right).
In the cluster of attribute questions, sub-clusters are mainly made by types of spatial relationship used to specify the target digit (\eg \#3 in Figure~\ref{fig:md_ex}), whereas sub-clusters in counting questions are based on whether the target digits of the question are selected from the targets of the previous question or not (\eg \#1 vs. \#2 in Figure~\ref{fig:md_ex}).

\vspace{-0.05cm}
Figure~\ref{fig:mdial_qualitative} illustrates qualitative results.
% We conduct a qualitative analysis on the effect of changes in retrieved attentions to the final attention calculation as illustrated in Figure~\ref{fig:mdial_qualitative}.
Based on the history of attentions stored in the attention memory, the proposed model retrieves the previous reference as presented in the second column.
The final attention for the current question is then calculated by manipulating the retrieved attention based on the current question.
For example, the current question in Figure~\ref{fig:mdial_qualitative} refers to the right digit of the previous reference, and the model identifies the target reference successfully (column~3) as the previous reference (column~2) is given accurately by the retrieved attention.
%
%\vspace{-0.05cm}
To investigate consistency with respect to attention manipulation,
% For the analysis, 
we move the region of the retrieved attention manually (column~4) and observe the final attention map calculated from the modified attention (column~5).
It is clear that our reference resolution procedure works consistently even with the manipulated attention and responds to the question accordingly. This shows a level of semantic interpretability of our model. 
See more qualitative results in Section~A of our supplementary material.
% We observe that the proposed model attends to different target references with different retrieved attentions while still preserving the semantics between the retrieved attentions and the final attentions.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/mdial_qualitative.pdf}
    \vspace{-0.1cm}
    \caption{
        {\bf Qualitative analysis on MNIST Dialog.} %  effect of retrieved attention to final attention calculation. 
        Given an input image and a series of questions with their visual grounding history, we present the memory retrieved and final attentions for the current question in the second and third columns, respectively.
        The proposed network correctly attends to target reference %by shifting the % relating to 
        %retrieved attention to the right % (right side of retrieved attention) 
        and predicts correct answer.
        The last two columns present the manually modified attention % to see effect of change in retrieved attention.
        and the final attention obtained from the modified attention, respectively. % which is also changed accordingly. 
        Experiment shows consistency of transformation between attentions and semantic interpretability of our model.
    }
    \label{fig:mdial_qualitative}
    \vspace{-0.1in}
\end{figure}

\vspace{-0.05cm}
\subsection{Visual Dialog (VisDial) Dataset}
\vspace{-0.1cm}
\paragraph{Experimental Setting}
% Moving to the experiments on a real dataset, we conduct the experiments on Visual Dialog (VisDial) introduced in \cite{visdial}.
In the VisDial \cite{visdial} dataset\footnote{We use recently released VisDial v0.9 with the benchmark splits \cite{visdial}.}, the dialogs are collected from MS-COCO~\cite{mscoco} images and their captions.
% It is built by collecting dialogs about images of MS-COCO~\cite{mscoco} with their captions.
% In VisDial, 
Each dialog is composed of an image, a caption, and a sequence of ten QA pairs.
Unlike in MNIST Dialog, answers to questions in VisDial are in free form text. % s with variable lengths.
Since each dialog always starts with an initial caption annotated in MS-COCO, the initial history is always constructed using the caption. %the history for a question always starts with the caption as the first element.
The dataset provides 100 answer candidates for each question and accuracy of a question is measured by the rank of the matching ground-truth answer. %models are evaluated based on the rank of the GT answer. % among them.
Note that this dataset is less focused on visual reference resolution and contains fewer % less number of 
ambiguous expressions compared to MNIST Dialog.
We estimate the portion of questions 
% the portion of sentences 
containing ambiguous expressions to be 94\% and 52\% in MNIST Dial and VisDial, respectively\footnote{We consider pronouns and definite noun phrases as ambiguous expressions and count them using a POS tagger in NLTK (\url{http://www.nltk.org/}).}.

While we compare our model with various encoders introduced in \cite{visdial}, we fix the decoder to a discriminative decoder that directly ranks the answer candidates through their embeddings. 
% without a generative process.
Our baselines include three visual dialog models, \ie late fusion model (LF), hierarchical recurrent encoder (HRE) and memory network encoder (MN), and two attention based VQA models (SAN and HieCoAtt) with the same decoder.
% of the three models attached.
The three visual dialog baselines are trained with different valid combinations of inputs, which are denoted by Q, I and H in the model names.


We perform the same ablation study of our model with the one for MNIST Dialog dataset.
%We build our full model that uses both the history embeddings and the sequential preference in addressing for the experiments on VisDial.
The \texttt{conv5} layer in VGG-16~\cite{VGG16} trained on ImageNet~\cite{ImageNet} is used to extract the image feature map.
Similar to~\cite{visdial}, all word embedding layers share their weights and an LSTM is used for embedding the current question.
For the models with history embedding, we use additional LSTMs for the questions, the answers, and the captions in the history. 
Based on our empirical observation, we share the  parameters of the question and caption LSTMs while having a separate set of weights for the answer LSTM.
%Also, we use a single LSTM for embedding the questions, the answers and the captions in the history, while a separate LSTM is used for embedding the current question.
Every LSTM embedding sentences is two-layered, but the history LSTM of HRNN has a single layer.
We employ 64 dimensional word embedding vectors  % activations 
and 128 dimensional hidden state for every LSTM. % in the model.
Note that the the dimensionality of our word embeddings and hidden state representations in LSTMs are significantly lower than the baselines (300 and 512 respectively).
We train the network using Adam~\cite{Adam} with the initial learning rate of 0.001 and weight decaying factor 0.0001. 
Note that we do not update the feature extraction network based on VGG-16.

\begin{table}[t]
    \centering
    \caption{{\bf Experimental results on VisDial.} We show the number of parameters, mean reciprocal rank (MRR), recall@$k$ and mean rank (MR). 
    +H and ATT indicate use of history embeddings in prediction and attention mechanism, respectively.
    }
    \vspace{0.05in} 
    \scalebox{0.85}{ 
        \begin{tabular}{
            p{3.5cm}@{}C{1cm}@{}@{}C{1cm}@{}@{}C{3.1cm}@{}@{}C{0.15cm}@{}@{}C{1.6cm}@{}@{}C{1.3cm}@{}@{}C{1.3cm}@{}@{}C{1.3cm}@{}@{}C{1.3cm}@{}
        }
            Model                       & +H            & ATT           & \# of params              && MRR       & R@1   & R@5   & R@10  & MR  \\ \toprule
            Answer prior \cite{visdial} & --            & --            & n/a                       && 0.3735    & 23.55 & 48.52 & 53.23 & 26.50 \\ \cmidrule(lr){1-10}
            LF-Q \cite{visdial}         & --            & --            & \phantom{0}8.3 M (3.6x)   && 0.5508    & 41.24 & 70.45 & 79.83 & 7.08  \\
            LF-QH \cite{visdial}        & \checkmark    & --            & 12.4 M (5.4x)             && 0.5578    & 41.75 & 71.45 & 80.94 & 6.74  \\
            LF-QI \cite{visdial}        & --            & --            & 10.4 M (4.6x)             && 0.5759    & 43.33 & 74.27 & 83.68 & 5.87  \\
            LF-QIH \cite{visdial}       & \checkmark    & --            & 14.5 M (6.3x)             && 0.5807    & 43.82 & 74.68 & 84.07 & 5.78  \\ \cdashlinelr{1-10}
            HRE-QH \cite{visdial}       & \checkmark    & --            & 15.0 M (6.5x)             && 0.5695    & 42.70 & 73.25 & 82.97 & 6.11  \\
            HRE-QIH \cite{visdial}      & \checkmark    & --            & 16.8 M (7.3x)             && 0.5846    & 44.67 & 74.50 & 84.22 & 5.72  \\
            HREA-QIH \cite{visdial}     & \checkmark    & --            & 16.8 M (7.3x)             && 0.5868    & 44.82 & 74.81 & 84.36 & 5.66  \\ \cdashlinelr{1-10}
            MN-QH \cite{visdial}        & \checkmark    & --            & 12.4 M (5.4x)             && 0.5849    & 44.03 & 75.26 & 84.49 & 5.68  \\
            MN-QIH \cite{visdial}       & \checkmark    & --            & 14.7 M (6.4x)             && 0.5965    & 45.55 & 76.22 & 85.37 & 5.46  \\ \cmidrule(lr){1-10}
            SAN-QI \cite{stackAtt}      & --            & \checkmark    & n/a                       && 0.5764    & 43.44 & 74.26 & 83.72 & 5.88  \\
            HieCoAtt-QI \cite{hierATT}  & --            & \checkmark    & n/a                       && 0.5788    & 43.51 & 74.49 & 83.96 & 5.84  \\ \cmidrule(lr){1-10}
            AMEM-QI                     & --            & \checkmark    & \bf1.7 M (0.7x)           && 0.6196    & 48.24 & 78.33 & 87.11 & 4.92  \\
            AMEM-QIH                    & \checkmark    & \checkmark    & 2.3 M (1.0x)              && 0.6192    & 48.05 & 78.39 & 87.12 & 4.88  \\
            AMEM+SEQ-QI                 & --            & \checkmark    & \bf1.7 M (0.7x)           && \bf0.6227 & \bf48.53 & \bf78.66 & \bf87.43 & \bf4.86  \\
            AMEM+SEQ-QIH                & \checkmark    & \checkmark    & 2.3 M (1.0x)              && 0.6210    & 48.40 & 78.39 & 87.12 & 4.92  \\ \bottomrule
        \end{tabular}
    }
    \label{tab:visdial_res}
    \vspace{-0.05in}
\end{table}

\vspace{-0.1in}
\paragraph{Results}
Table~\ref{tab:visdial_res} presents mean reciprocal rank (MRR), mean rank (MR), and recall@$k$ of the models.
Note that lower is better for MRs but higher is better for all other evaluation metrics.
All variants of the proposed model outperform the baselines in all metrics, achieving the state-of-the-art performance.
As observed in the experiments on MNIST Dialog, the models with sequential preference (+SEQ) show better performances compared to the ones without it. 
However, we do not see additional benefits from using a history embedding on VisDial, in contrast to MNIST Dialog.
%\brk{our history embedding by HRNN fails to extract additional information of dialog structure other than the one stored in the memory.}
The proposed algorithm also has advantage over existing methods in terms of the number of parameters.
Our full model only requires approximately 15\% of parameters compared to the best baseline model without counting the parameters in the common feature extraction module based on VGG-16.
In VisDial, the attention based VQA techniques with (near) state-of-the-art performances are not as good as the baseline models of~\cite{visdial} because they treat each question independently.
The proposed model improves the performance on VisDial by facilitating the visual reference resolution process.
Qualitative results for VisDial dataset are presented in Section~B of the supplementary material.
% 

==> NIPS 2017 Camera ready/sections/introduction.tex <==
% !TEX root = ../nips_2017.tex

\section{Introduction}
%Recap
In recent years, % advancements 
advances in the design and optimization of deep neural network architectures have led to tremendous progress across many areas of computer vision (CV) and natural language processing (NLP). 
This progress, in turn, has enabled a variety of multi-modal applications
% and have allowed applications to a variety of multi-modal tasks 
spanning both domains, including image captioning~\cite{showtell,showAtt,muncaption}, language grounding~\cite{refres,refres2}, image generation from captions~\cite{imgen1,imgen2}, and visual question answering (VQA) on images~\cite{DPPNet,stackAtt,askAtt,compQA,snuAtt,NMN,hierATT,multiBilin,hyunwooVQA,VQA,VQA2,BBVQA,Askneurons} and videos~\cite{marioQA,VideoQA,MovieQA}.

%VQA task: Why is it important? How is it approached?
The VQA task, in particular, has received broad attention because its formulation requires a universal understanding of image content. 
Most state-of-the-art methods~\cite{snuAtt,stackAtt,hierATT} address this inherently challenging problem through an attention mechanism~\cite{showAtt} that allows to visually ground linguistic expressions; they identify the region of visual interest referred to by the question and predict the answer based on the visual information in that region. 

%Visual dialog task: How does it differ from VQA? What are the additional challenges?
More recently, Visual Dialog~\cite{visdial} has been introduced as a generalization of the VQA task. Unlike VQA, where every question is asked independently, a visual dialog system needs to answer a \emph{sequence} of questions about an input image. 
The sequential and inter-dependent property of questions in a dialog presents additional challenges.
%
Consider the simple image and partial dialog in Figure~\ref{fig:md_ex}. 
Some questions (\eg \#1: `How many 9's are there in the image?') contain the full information needed to attend to the regions within the image and answer the question accurately. 
Other questions (\eg \#6: `What is the number of the blue digit?') are ambiguous on their own and require knowledge obtained from the prior questions (1, 2, 3, and 5 in particular) in order to resolve attention to the specific region the expression (`the blue digit') is referring to.  
This process of \emph{visual reference resolution}\footnote{We coin this term by borrowing nomenclature, partially, from NLP, where coreference resolution attempts to solve the corresponding problem in language; the {\em visual} in {\em visual reference resolution} implies that we want to do both resolve and visually ground the reference used in the question.} is the key component required to localize attention accurately in the presence of ambiguous expressions and thus plays a crucial role in extending VQA approaches to the visual dialog task.

% When computing an attention, each question must therefore be viewed in the context of the dialog history in order to resolve ambiguous expressions caused by the question's sequential dependencies (e.g., `Where is it?' must be resolved to the object `it' is referring to in order to obtain the correct attention.). This process of \emph{visual reference resolution} is the key in obtaining clean attentions in the presence of ambiguous expressions and thus in extending VQA approaches to the visual dialog task in general.\footnote{Figure 1 is very in-depth. It might be good to add a high-level Figure to the top of page 2 that can be referred to in the introduction. Basically a Figure explaining the task, the terms `visual reference resolution'/`ambiguous expression'/`sequential dependency' and how they affect the attentions.}

%Approach: How do we tackle those challenges?
We perform visual reference resolution relying on a novel attention mechanism that employs an associative memory to obtain a visual reference for an ambiguous expression. The proposed model utilizes two types of intermediate attentions: tentative and retrieved ones. 
The {\em tentative attention} is calculated solely based on the current question (and, optionally, the dialog history), and is capable of focusing on an appropriate region when the question is unambiguous. 
The {\em retrieved attention}, used for visual reference resolution, is the most relevant previous attention available  in the associative memory. 
The final attention for the current question is obtained by combining the two attention maps conditioned on the question; this is similar to neural module networks~\cite{NMN,compQA}, which dynamically combine discrete attention modules, based on a question, to produce the final attention. %, our model dynamically adjusts the parameters of the combining attention module. 
For this task, our model adopts a dynamic parameter layer~\cite{DPPNet} that allows us to work with continuous space of dynamic parametrizations, as opposed to the discrete set of parametrizations in~\cite{NMN,compQA}.

%Similar to neural module networks~\cite{NMN,compQA}, which change the parameters of modules depending on the input word to combine attentions adaptively, our model adjusts the parameters of the combining module of attentions based on the question.
%\hsseo{Our model adopt a dynamic parameter layer~\cite{DPPNet} as it should maintain parameters for questions represented as contiguous embeddings.}

%\leon{[I don't really understand the last sentence]}
%The final attention for the current question is obtained by combining the two attentions using a dynamic parameter prediction network~\cite{DPPNet}. %{\color{red}[We should clarify here why we need {\em dynamic} parameter prediction.]}


%Contributions
\paragraph{Contributions} We make the following contributions. (1) We introduce a novel attention process that, in addition to direct attention, resolves visual references % of questions with ambiguous expressions 
by modeling the sequential dependency of the current question on previous attentions through an associative attention memory; (2) We perform a comprehensive analysis of the capacity of our model for the visual reference resolution task using a synthetic visual dialog dataset (MNIST dialog) and obtain superior performance compared to all baseline models.
%We provide comprehensive experiments on a synthetic visual dialog dataset to analyze the capacity of our model for visual reference resolution task and show that the proposed model outperforms all baseline models; 
(3) We test the proposed model in a visual dialog benchmark (VisDial~\cite{visdial}) and show state-of-the-art performance with significantly fewer parameters.

%a very small number of activations for sentence embeddings.

\begin{figure}
    \centering
    \scalebox{0.8}{
    \includegraphics{figures/mdial_ex.jpg}~~~~~~~~~~~
    \begin{tabular}[b]{cp{7.8cm}c}
    \# & Question                                                     & Answer \\ \hline
    1 & How many 9's are there in the image?                         & four \\
    2 & How many brown digits are there among them?                  & one \\
    3 & What is the background color of the digit at the left of it? & white \\
    4 & What is the style of the digit?                              & flat \\
    5 & What is the color of the digit at the left of it?            & blue \\
    6 & What is the number of the blue digit?                        & 4 \\
    7 & Are there other blue digits?                                 & two
    \end{tabular}
    }
    \caption{{\bf Example from MNIST Dialog.} Each pair consists of an image (left) and a set of sequential questions with answers (right).}
    \label{fig:md_ex}
    \vspace{-0.1in}
\end{figure}

==> NIPS 2017 Camera ready/sections/model.tex <==
% !TEX root = ../nips_2017.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{./figures/network_architecture.pdf}
%     \caption{Architecture of the entire proposed network. Letters in parentheses are to label each module of network described in Section~\ref{model}. Note that gray box represents module described in Section~\ref{attmem}.}
%     \label{fig:network_architecture}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Additional Components and Implementation}
% \section{Neural Model with Reference Resolution for Visual Dialog}
\label{model}

In addition to the attended image feature, we find other information useful for answering the question. Therefore, for the final encoding $\bm{e}_t$ at time step $t$, we fuse the attended image feature embedding $\bm{f}^\mathrm{att}_t$ with the context embedding $\bm{c}_t$, the attention map $\bm{\alpha}_t$ and the retrieved key $\bm{k}^\mathrm{mem}_t$ from the memory, by a \texttt{fc} layer after concatenation (Figure~\ref{fig:network_architecture}f).
    
Finally, when we described the associative memory in Section~\ref{attmem}, we did not specify the memory key generation procedure. In particular, after answering the current question, we append the computed attention map to the memory.
% (to be used by subsequent questions). 
When storing the current attention into  memory, the proposed model generates a key $\bm{k}_t$ by fusing the context embedding $\bm{c}_t$ with the current answer embedding $\bm{a}_t$ through a \texttt{fc} layer (Figure~\ref{fig:network_architecture}h).
Note that an answer embedding $\bm{a}_t$ is obtained using LSTM.

% In addition to the components described in Section~\ref{attmem}, the proposed model consists of the following modules as depicted in Figure~\ref{fig:network_architecture}.

% \begin{itemize}[leftmargin=0cm,label={}]
%    \item {\bf Question embedding}
%    We use a recurrent neural network (RNN) with long-short term memory (LSTM) units to encode the current input question (Figure~\ref{fig:network_architecture}a).
%    
%    \item {\bf History embedding}
%    A hierarchical RNN (HRNN) structure with LSTMs is used to embed history information  (Figure~\ref{fig:network_architecture}b).
%    The questions and the answers of a history are independently embedded by LSTM-RNNs and then fused by a \texttt{fc} layer with concatenation to form QA embeddings.
%    The fused QA embedding at each time step is finally fed to another LSTM-RNN and the final output is used for the history embedding.
%    
%    \item{\bf Image feature extraction}
%    A convolutional neural network (CNN) is used to extract a feature map from the input image (Figure~\ref{fig:network_architecture}c). 
%    The same feature map is shared at every time step of a dialog.
%    
%   \item{\bf Attended image feature embedding}
%    As described in Section~\ref{attmem}, we use an encoder module that embeds images with attention by resolving a visual reference using previous attentions stored in the attention memory  (Figure~\ref{fig:network_architecture}e).
%    We extend this module by replacing the question embedding $c_t$ in Section~\ref{attmem} with the mixture of the question and the history embeddings $\tilde{c}_t$, which is called a context embedding and is computed by a \texttt{fc} layer with the concatenation of the two embeddings  (Figure~\ref{fig:network_architecture}d).
%     
%     \item{\bf Multimodal feature encoder}
%     In addition to the attended image feature, there are other information useful for answering the question.
%     Thus, for the final encoding $e_t$ at time step $t$, we fuse the attended image feature embedding $f^\mathrm{att}_t$ with the context embedding $\tilde{c}_t$, the attention map $\alpha_t$ and the retrieved key $k^\mathrm{mem}_t$ from the memory by a \texttt{fc} layer after concatenation (Figure~\ref{fig:network_architecture}f).
    
 %   \item{\bf Answer decoder}
 %   After encoding the inputs into a single vector $e_t$, the proposed model decodes the answer from it (Figure~\ref{fig:network_architecture}g).
 %   We choose different decoders depending on the dataset.
%     
%     \item{\bf Memory key generation}
%     After answering current question, we append the computed attention map to the memory for next questions.
%     When storing the current attention to the memory, the proposed model generates a key $k_t$ by fusing the context embedding $\tilde{c}_t$ with the current answer embedding $a_t$ through a \texttt{fc} layer (Figure~\ref{fig:network_architecture}h).
%     Note that an answer embedding $a_t$ is obtained by an LSTM-RNN.
    
% \end{itemize}

\vspace{-0.1in}
\paragraph{Learning} Since all the modules of the proposed network are fully differentiable, the entire network can be trained end-to-end by standard gradient-based learning algorithms.

==> NIPS 2017 Camera ready/sections/related_work.tex <==
% !TEX root = ../nips_2017.tex

\section{Related Work}

\paragraph{Visual Dialog}
Visual dialogs were recently proposed in \cite{visdial} and \cite{guesswhat}, focusing on different aspects of a dialog. While the conversations in the former contain free-form questions about arbitrary objects, the dialogs in the latter aim at object discovery through a series of yes/no questions. 
Reinforcement learning (RL) techniques were built upon those works in \cite{visdialRL} and \cite{guesswhatRL}. 
Das et al.~\cite{visdialRL} train two agents by playing image guessing games and show that they establish their own communication protocol and style of speech. In~\cite{guesswhatRL}, RL is directly used to improve the performance of agents in terms of the task completion rate of goal-oriented dialogs. 
%Besides these works, 
However, the importance of previous references has not yet been explored in the visual dialog task.

\paragraph{Attention for Visual Reference Resolution}
%{\color{red}[Many sentences in this paragraph is more appropriate to introduction section.] 
While visual dialog is a recent task, VQA has been studied extensively and attention models have been known to be beneficial for answering independent questions~\cite{askAtt,stackAtt,snuAtt,compQA,NMN,hierATT,multiBilin}. 
However, none of those methods incorporate visual reference resolution, which is neither necessary nor possible in VQA but essential in visual dialog.
Beyond VQA, attention models are used to find visual groundings of linguistic expressions in a variety of other multi-modal tasks, such as image captioning~\cite{muncaption,showAtt}, VQA in videos~\cite{marioQA}, and visual attributes prediction~\cite{PAN}. 
Common to most of these works, an attention is obtained from a single embedding of all linguistic inputs. 
Instead, we propose a model that embeds each question in a dialog separately and calculates the current question's attention by resolving its sequential dependencies through an attention memory and a dynamic attention combination process.
We calculate an attention through a dynamic composition process taking advantage of a question's semantic structure, which is similar  to~\cite{compQA} and~\cite{NMN}.
However, the proposed method still differs in that our attention process is designed to deal with ambiguous expressions in dialogs by dynamically analyzing the dependencies of questions at each time step. In contrast, \cite{compQA} and~\cite{NMN} obtain the attention for a question based on its compositional semantics that is completely given at the time of the network structure prediction.
%However, we differ from those approaches in several key aspects: (1) The sequential dependency is dynamically analyzed at each time step through memory retrieval, unlike previous works, which require the entire semantics at the time of the network structure prediction; (2) Our attention process is designed to deal with ambiguous expressions in dialogs, whereas the attentions in~\cite{NMN,compQA} are used to resolve a question's grounding based on compositional semantics; (3) Finally, our model predicts the parameters of the attention combination module dynamically from embeddings in a continuous space and can therefore accept infinitely many possible sentences; the sub-modules in the previous works are formed based on finite words.}

\paragraph{Memory for Question Answering}
Another line of closely related works is the use of a memory component to question answering models.
Memory networks with end-to-end training are first introduced in \cite{memn2n}, extending the original memory network~\cite{memNet}.
The memories in these works are used to store some factoids in a given story and the supporting facts for answering questions are selectively retrieved through memory addressing.
A memory network with an episodic memory was proposed in~\cite{dmnorg} and applied to VQA by storing the features at different locations of the memory \cite{dmnvqa}.
While these memories use the contents themselves for addressing, \cite{keymem} proposes associative memories that have a key-value pair at each entry and use the keys for addressing the value to be retrieved.
Finally, the memory component is also utilized % facilitated
for visual dialog in \cite{visdial} to actively select the previous question in the history.
Memories in these previous memory networks store given factoids to retrieve a supporting fact.
In contrast, our attention memory stores previous attentions, which represent grounded references for previous questions, to resolve the current reference based on the sequential dependency of the referring expressions.
Moreover, we adopt an associative memory to use the semantics of QA pairs for addressing. % because the attentions alone cannot represent their semantics.


